Generalized Sparse Additive Models

We present a unified framework for estimation and analysis of generalized additive models in high dimensions. The framework defines a large class of penalized regression estimators, encompassing many existing methods. An efficient computational algorithm for this class is presented that easily scales to thousands of observations and features. We prove minimax optimal convergence bounds for this class under a weak compatibility condition. In addition, we characterize the rate of convergence when this compatibility condition is not met. Finally, we also show that the optimal penalty parameters for structure and sparsity penalties in our framework are linked, allowing cross-validation to be conducted over only a single tuning parameter. We complement our theoretical results with empirical studies comparing some existing methods within this framework.

==> sections/app_proofBig.tex <==


\section{Proofs of Results in Section \ref{sec:main}}
In this section we present the proof Theorem~\ref{thm:main1} and \ref{thm:main2} for the sake of completeness. The arguments presented here are only a slight modification to those of \cite{buehlmann2011statistics} for proving LASSO rates. One notable difference is that we explicitly handle an unpenalized intercept term; another is our handling of the structural penalty, $P_{st}(\cdot)$. Throughout the proofs, we will utilize the so-called \textit{basic inequalities}. Hence, for the sake of convenience, we state and prove these basic inequalities as a separate lemma.
\begin{lemma}[Basic Inequality]
\label{lemma:basicIneq}
Let $\wh{f}(\bs{x}) = \wh{\beta} + \sum_{j=1}^{p}\wh{f}_j(x_{j})$ be as defined in \eqref{eq:prop}, and let $f^*(\bs{x}) = \beta^* + \sum_{j=1}^{p}f_j^*(x_j)$ be an arbitrary additive function with $\beta^*\in \mathcal{R}$ and $f_j^*\in \mathcal{F}$. Then we have the following basic inequality
\begin{equation}
\label{eqn:basic1}
\mathcal{E}(\wh{f})  + \lambda I(\wh{f}) \le - \left[ \nu_n(\wh{f}) - \nu_n(f^*) \right] + \lambda I(f^*) + \mathcal{E}(f^*).
\end{equation} 
If we further assume that $-\ell(\cdot)$ and $P_{st}(\cdot)$ are convex, then for all $t\in (0,1)$ and $\wt{f} = t\wh{f} + (1-t)f^*$ we have the following basic inequality
\begin{equation}
\label{eqn:basic2}
\mathcal{E}(\wt{f})  + \lambda I(\wt{f}) \le - \left[ \nu_n(\wt{f}) - \nu_n(f^*) \right] + \lambda I(f^*) + \mathcal{E}(f^*).
\end{equation} 
\end{lemma}
%We will later specify a specific choice for $f^*$ which will be referred to as the \textit{oracle}. To study the local behavior of the empirical process we define $Z_M$ as follows:
%\begin{equation}
%\label{eqn:Z_M}
%Z_M = \underset{I(f - f*)\le M}{\sup } \left| \nu_n(f)  - \nu_n(f^*) \right|.
%\end{equation}
\begin{proof}
For the first inequality, note that
\begin{align*}
-\mathbb{P}_n \ell\left(\wh{f}\right) + \lambda I(\wh{f}) \le -\mathbb{P}_n \ell\left({f^*}\right) + \lambda I({f}^*),
\end{align*}
which is equivalent to 
\begin{align*}
&\  \ \ \ \  \lambda I(\wh{f}) \le \mathbb{P}_n \ell\left(\wh{f}\right) - \mathbb{P}_n \ell\left({f^*}\right) + \lambda I({f}^*)\\
&\Leftrightarrow   \mathbb{P}(\ell({f}^*))- \mathbb{P}(\ell(\wh{f})) + \lambda I(\wh{f}) \le \mathbb{P}_n \ell\left(\wh{f}\right) - \mathbb{P}(\ell(\wh{f})) - \mathbb{P}_n \ell\left({f^*}\right) + \mathbb{P}(\ell({f}^*)) + \lambda I({f}^*)\\
&\Leftrightarrow   \mathbb{P}(\ell({f}^*))- \mathbb{P}(\ell(\wh{f})) + \lambda I(\wh{f}) \le - \left[(\mathbb{P}_n- \mathbb{P})(-\ell(\wh{f})) - (\mathbb{P}_n- \mathbb{P})(-\ell(f^*))\right] + \lambda I({f}^*)\\
&\Leftrightarrow   \mathbb{P}(\ell({f}^*))- \mathbb{P}(\ell(\wh{f})) + \lambda I(\wh{f}) \le - \left[\nu_n(\wh{f}) - \nu_n(f^*)\right] + \lambda I({f}^*)\\
&\Leftrightarrow   \mathbb{P}(\ell({f}^*)) -\mathbb{P}(\ell(f^0)) + \mathbb{P}(\ell(f^0))- \mathbb{P}(\ell(\wh{f})) + \lambda I(\wh{f}) \le - \left[\nu_n(\wh{f}) - \nu_n(f^*)\right] + \lambda I({f}^*)\\
&\Leftrightarrow   -\mathcal{E}(f^*) + \mathcal{E}(\wh{f}) + \lambda I(\wh{f}) \le - \left[\nu_n(\wh{f}) - \nu_n(f^*)\right] + \lambda I({f}^*).
\end{align*}
For the second inequality we have by convexity
\begin{align*}
-\mathbb{P}_n \ell\left(\wt{f}\right) + \lambda I(\wt{f}) &\le t\left[-\mathbb{P}_n \ell\left(\wh{f}\right) + \lambda I(\wh{f})\right] + (1-t)\left[ -\mathbb{P}_n \ell\left({f^*}\right) + \lambda I({f^*}) \right]\\
&\le  -\mathbb{P}_n \ell\left({f^*}\right) + \lambda I({f^*}),
\end{align*}
after which we simply need to repeat the arguments for the previous basic inequality with $\wh{f}$ replaced by $\wt{f}$. 
\end{proof}


\begin{proof}[\textbf{Proof of Theorem~\ref{thm:main1}}]
Define 
\begin{equation}
\label{eqn:tVal}
t = \frac{M^* }{M^* + I(\wh{f} - f^*)},
\end{equation}
and $\wt{f} = t\wh{f} + (1-t)f^*$. Then \eqref{eqn:tVal} implies $I(\wt{f} - f^*) \le M^*$ and by Lemma~\ref{lemma:basicIneq}, we obtain 
\begin{equation*}
\mathcal{E}(\wt{f}) +  \lambda I(\wt{f}) \le Z_{M^*} + \lambda I(f^*) + \mathcal{E}(f^*).
\end{equation*} 
By applying the triangle inequality $I(\wt{f}-f^* + f^*)\ge I(\wt{f} - f^*) - I(f^*)$, to the left hand side we obtain on the set $\mathcal{T}$ (where $Z_{M^*} \le \rho M^* + 2R\rho$)
\begin{align*}
\mathcal{E}(\wt{f}) +  \lambda I(\wt{f}-f^*) \le \rho M^*  + 2R\rho + 2\lambda I(f^*) + \mathcal{E}(f^*).
\end{align*}
Recall the definition of $M^*$, given by 
\begin{equation}
\rho M^* = \mathcal{E}(f^*) + 2\lambda I(f^*) + 2R\rho,
\end{equation}
from which we obtain 
\begin{align*}
\mathcal{E}(\wt{f}) +  \lambda I(\wt{f}-f^*) \le 2\rho M^* \le 2\frac{\lambda }{4}M^* \Rightarrow I(\wt{f} - f^*)\le \frac{M^*}{2}.
\end{align*}
Now by the definition of $\wt{f}$ we have 
\begin{align*}
I(\wh{f} - f^*) = \frac{I(\wt{f} - f^*)}{t} = I(\wt{f} - f^*)\left[ 1 + \frac{I(\wh{f} - f^*)}{M^*} \right] \le \frac{M^*}{2} + \frac{I(\wh{f} - f^*)}{2},
\end{align*}
which implies that $I(\wh{f} - f^*)\le M^*$. Now we can repeat the above arguments with $\wt{f}$ replaced by $\wh{f}$ which gives us 
\begin{equation*}
\mathcal{E}(\wh{f}) +  \lambda I(\wh{f}-f^*) \le \rho M^* + \rho(2R) + 2\lambda I(f^*) + \mathcal{E}(f^*).
\end{equation*}
\end{proof}

% % % BEGIN PROOF FOR FAST RATES % % % %
% % % BEGIN PROOF FOR FAST RATES % % % %
% % % BEGIN PROOF FOR FAST RATES % % % %
% % % BEGIN PROOF FOR FAST RATES % % % %
\begin{proof}[\textbf{Proof of Theorem~\ref{thm:main2}}]
As in the proof of Theorem~\ref{thm:main1}, we begin by defining $t$ as 
\begin{equation*}
t = \frac{M^*}{M^* + |\wh{\beta} - \beta^*| + I(\wh{f} - f^*)},
\end{equation*}
and $\wt{f} = t\wh{f} + (1-t)f^*$ which gives us $|\wt{\beta} - \beta^*| + I(\wt{f} - f^*) \le M^*$, i.e. $\wt{f}\in \mathcal{F}^0_{local}$. Lemma~\ref{lemma:basicIneq} implies that on the set $\mathcal{T}$~(where $Z_{M^*}\le \rho M^*$) we have
\begin{equation}
\label{eqn:Ineq-slow1}
\mathcal{E}(\wt{f}) + \lambda I(\wt{f}) \le Z_{M^*} + \mathcal{E}^* + \lambda I(f^*) \le \rho M^*+ \mathcal{E}(f^*) + \lambda I(f^*).
\end{equation}
Be definition of $S_*$ and $I(\cdot)$, we have by the triangle inequality
\begin{align*}
\lambda I({f}^*) &=  \lambda \sum_{j\in S_*}\Big\{ \|f_j^*\|_n + \lambda P_{st}(f_j^*) \Big\} \le \lambda \sum_{j\in S_*}\Big\{ \|f_j^* - \wt{f}_j\|_n + \|\wt{f}_j\|_n+ \lambda P_{st}(f_j^*) \Big\},
\end{align*} 
and by the reverse triangle inequality we have
\begin{align*}
\lambda I(\wt{f}) &= \lambda \sum_{j\in S_*} \Big\{  \|\wt{f}_j\|_n + \lambda P_{st}(\wt{f}_j) \Big\} + \lambda \sum_{j\in S_*^c} \Big\{  \|\wt{f}_j\|_n + \lambda P_{st}(\wt{f}_j) \Big\}\\
&\ge \lambda \sum_{j\in S_*} \Big\{  \|\wt{f}_j\|_n + \lambda P_{st}(\wt{f}_j - f_j^*) - \lambda P_{st}(f_j^*) \Big\} + \lambda \sum_{j\in S_*^c} \Big\{  \|\wt{f}_j\|_n + \lambda P_{st}(\wt{f}_j) \Big\}\\
&= \lambda \sum_{j\in S_*} \Big\{  \|\wt{f}_j\|_n + \lambda P_{st}(\wt{f}_j - f_j^*) - \lambda P_{st}(f_j^*) \Big\} + \lambda \sum_{j\in S_*^c} \Big\{  \|\wt{f}_j - f_j^*\|_n + \lambda P_{st}(\wt{f}_j - f_j^*) \Big\},
\end{align*}
where the last equality follows from the fact that $f_j^* = 0 $ for all $j\in S_*^c$. With the above two inequalities combined with \eqref{eqn:Ineq-slow1} we get 
\begin{align*}
\mathcal{E}(\wt{f}) + &\lambda \sum_{j\in S_*} \Big\{  \|\wt{f}_j\|_n + \lambda P_{st}(\wt{f}_j - f_j^*) - \lambda P_{st}(f_j^*) \Big\} + \lambda \sum_{j\in S_*^c} \Big\{  \|\wt{f}_j\|_n + \lambda P_{st}(\wt{f}_j) \Big\}\\
 \le &\lambda \sum_{j\in S_*}\Big\{ \|f_j^* - \wt{f}_j\|_n + \|\wt{f}_j\|_n+ \lambda P_{st}(f_j^*) \Big\} + \rho M^* + \mathcal{E}(f^*),
\end{align*}
which simplifies to 
\begin{equation}
\label{eqn:Ineq-fast1}
\mathcal{E}(\wt{f}) +  \lambda\sum_{j\in S^c_*}\|\wt{f}_j - f_j^*\|_n  + \lambda \sum_{j=1}^p  \lambda P_{st}(\wt{f}_j - f_j^*)
 \le \lambda \sum_{j\in S_*} \|f_j^* - \wt{f}_j\|_n + 2\lambda^2\sum_{j\in S_*} P_{st}(f_j^*) + \rho M^* + \mathcal{E}(f^*).
\end{equation}
Now we add $\lambda|\wt{\beta} - \beta^*| + \lambda\sum_{j\in S_*} \|\wt{f}_j - f_j^*\|_n$ to both sides of \eqref{eqn:Ineq-fast1} to obtain 
\begin{equation}
\label{eqn:Ineq-fast2}
\mathcal{E}(\wt{f}) +  \lambda \Big\{ |\wt{\beta} - \beta^*| +  I(\wt{f} - f^*) \Big\} 
 \le 2\lambda \sum_{j\in S_*} \|f_j^* - \wt{f}_j\|_n  + \lambda|\wt{\beta} - \beta^*|+ \rho M^* + \mathcal{E}(f^*) + 2\lambda^2\sum_{j\in S_*} P_{st}(f_j^*).
\end{equation}

\noindent\textbf{Case I.} If 
\begin{equation*}
2\lambda \sum_{j\in S_*} \|f_j^* - \wt{f}_j\|_n  + \lambda|\wt{\beta} - \beta^*|\le \rho M^* + \mathcal{E}(f^*) + 2\lambda^2\sum_{j\in S_*} P_{st}(f_j^*),
\end{equation*}
then \eqref{eqn:Ineq-fast2} simplifies to 
\begin{align*}
\mathcal{E}(\wt{f}) +  \lambda \Big\{ |\wt{\beta} - \beta^*| +  I(\wt{f} - f^*) \Big\} 
&\le 2\rho M^* + 2\mathcal{E}(f^*) + 4\lambda^2\sum_{j\in S_*} P_{st}(f_j^*)\\
 &\le 4\rho M^* \le 4\frac{\lambda}{8}M^* = \lambda M^*/2, 
\end{align*}
which indicates that $|\wt{\beta} - \beta^*| +  I(\wt{f} - f^*) \le M^*/2$ which implies that $|\wh{\beta} - \beta^*| +  I(\wh{f} - f^*) \le M^*$ and hence we can redo the above arguments and replace $\wt{f}$ by $\wh{f}$.\newline

\noindent\textbf{Case II.} If instead 
\begin{equation*}
2\lambda \sum_{j\in S_*} \|f_j^* - \wt{f}_j\|_n  + \lambda|\wt{\beta} - \beta^*|\ge \rho M^* + \mathcal{E}(f^*) + 2\lambda^2\sum_{j\in S_*} P_{st}(f_j^*),
\end{equation*}
then we have 
\begin{align}
\label{eqn:Ineq-fast-case2}
\mathcal{E}(\wt{f}) +  \lambda \Big\{ |\wt{\beta} - \beta^*| +  I(\wt{f} - f^*) \Big\} 
&\le 4\lambda \sum_{j\in S_*} \|f_j^* - \wt{f}_j\|_n  + 2\lambda|\wt{\beta} - \beta^*|.
\end{align}
This is equivalent to 
\begin{align*}
\mathcal{E}(\wt{f}) +  \lambda \Big\{ \sum_{j\in S_*^c}\|\wt{f}_j - f_j^*\|_n + \lambda \sum_{j=1}^pP_{st}(\wt{f}_j-f_j^*)  \Big\} 
&\le 3\lambda \sum_{j\in S_*} \|f_j^* - \wt{f}_j\|_n  + \lambda|\wt{\beta} - \beta^*|,
\end{align*}
which means we have that 
\begin{equation*}
\sum_{j\in S_*^c}\|\wt{f}_j - f_j^*\|_n + \lambda \sum_{j=1}^pP_{st}(\wt{f}_j-f_j^*)  \le 3\sum_{j\in S_*}\|f_j^* - \wt{f}_j\|_n + |\wt{\beta} - \beta^*|,
\end{equation*}
and hence by the compatibility condition \eqref{eqn:Ineq-fast-case2} reduces to
\begin{align}
\mathcal{E}(\wt{f}) +  \lambda \Big\{ |\wt{\beta} - \beta^*| +  I(\wt{f} - f^*) \Big\} 
&\le 4\lambda \|\wt{f} - f^*\|\sqrt{s_*}/\phi(S_*).
\end{align}
Since $\wt{f}$ and $f^*$ are in $\mathcal{F}^0_{local}$, we invoke the inequality $uv\le H(v) + G(u)$ to obtain
\begin{align*}
\frac{4\lambda\sqrt{s_*}\|\wt{f} - f^*\|}{\phi(S_*)} &\le \frac{8\lambda\sqrt{s_*}}{\phi(S_*)} \left[ \frac{\|\wt{f} - f^0\|}{2} + \frac{\|{f}^* - f^0\|}{2} \right]\\
&\le H\left( \frac{8\lambda\sqrt{s_*}}{\phi(S_*)} \right) + G\left( \frac{\|\wt{f} - f^0\|}{2} + \frac{\|{f}^* - f^0\|}{2} \right).
\end{align*}
By the convexity of $G$ and the margin condition we obtain 
\begin{align*}
\frac{4\lambda\sqrt{s_*}\|\wt{f} - f^*\|}{\phi(S_*)} &\le H\left( \frac{8\lambda\sqrt{s_*}}{\phi(S_*)} \right) + \frac{\mathcal{E}(\wt{f})}{2} + \frac{\mathcal{E}({f}^*)}{2}.
\end{align*}
Hence we have 
\begin{align}
\frac{\mathcal{E}(\wt{f})}{2} +  \lambda \Big\{ |\wt{\beta} - \beta^*| +  I(\wt{f} - f^*) \Big\} 
&\le H\left( \frac{8\lambda\sqrt{s_*}}{\phi(S_*)} \right) + \frac{\mathcal{E}(f^*)}{2} \le \rho M^* \le \lambda M^*/8,
\end{align}
which implies that $|\wt{\beta} - \beta^*| +  I(\wt{f} - f^*) \le M^*/2$ which in turn implies $|\wh{\beta} - \beta^*| +  I(\wh{f} - f^*) \le M^*$ and hence we can redo the above arguments and replace $\wt{f}$ by $\wh{f}$.


Thus we have shown that 
\begin{align}
\mathcal{E}(\wh{f}) +  \lambda \Big\{ |\wh{\beta} - \beta^*| +  I(\wh{f} - f^*) \Big\} 
&\le 4\rho M^*.
\end{align}

\end{proof}



\section{The Set $\mathcal{T}$}
Theorems~\ref{thm:main1} and \ref{thm:main2a} show inequalities holding over the set $\mathcal{T}$. In this section we will show that $\mathcal{T}$ occurs with high probability. This will be shown for the two different types of entropy bounds considered in Section~\ref{sec:TheoreticalResults}. We consider the special case of loss functions linear in $Y_i$ as in Corollaries~\ref{cor:slowRates} and \ref{cor:fastrates} and bound the term $\nu_n(f) - \nu_n(f^*)$ in the following theorem.

\begin{theorem}
\label{lemma:Emp-Process}
Let $\bs{x}_i\in \mathbb{R}^p$ and $Y_i\in \mathbb{R}$ denote the fixed covariates and response, respectively, for $i=1,\ldots,n$. Assume that for any function $f$ the loss $\ell(\cdot)$ is such that 
\begin{equation}
-\ell(f) = -\ell(f, \bs{x}_i,Y_i) = aY_if(\bs{x}_i) + b(f(\bs{x}_i)),
\end{equation}
for some $a\in \mathbb{R}\backslash \{0 \}$ and function $b:\mathbb{R}\to \mathbb{R}$. Further assume that $Y_i - \mathbb{E}Y_i = Y_i - \mu_i$ are uniformly sub-Gaussian, i.e. 
\begin{equation}
\label{eqn:subGaussian}
\max_{i=1,\ldots,n} K^2\left( \mathbb{E}e^{(Y_i-\mu_i)^2/K^2} - 1 \right) \le \sigma_0^2,
\end{equation}
then with probability at-least $1-2\exp\left[ -n\rho^2C_1 \right] - C\exp\left[ -n\rho^2C_2 \right]$ the following inequality holds
\begin{equation}
\label{eqn:inequal-EmpiricalProcess}
\nu_n(f) - \nu_n(f^*) \le \rho\left[ |\beta-\beta^*| + \sum_{j=1}^{p}\|f_j-f_j^*\|_n + \lambda P_{st}(f_j-f_j^{*})\right],
\end{equation}
for variables $\rho,\, \lambda$ and positive constants $C,\, C_1,\,C_2$ which we specify in the following 3 cases.

\noindent\textbf{Case 1.} If $\mathcal{F}$ has a logarithmic entropy bound, then the inequality \eqref{eqn:inequal-EmpiricalProcess} holds with
$\rho = \kappa \max\left( \sqrt{\frac{T_n}{n}}, \sqrt{\frac{\log p}{n}} \right)$ and $\lambda = 1$ for constants $\kappa = \kappa(a,\, K,\, \sigma_0,\, A_0)$, $C_1 = C_1(K,\sigma_0)$, $C = C(K,\, \sigma_0)$ and $C_2 = C_2(C,\, \kappa)$.

\noindent\textbf{Case 2.} If $\mathcal{F}$ has a polynomial entropy bound with smoothness, then the inequality \eqref{eqn:inequal-EmpiricalProcess} holds with $\rho = \kappa \max\left( n^{-\frac{1}{2+\alpha}}, \sqrt{\frac{\log p}{n}} \right)$ for constants $\kappa = \kappa(a,\, K,\, \sigma_0,\, A_0,\, \alpha)$, $C_1 = C_1(K,\sigma_0)$, $C = C(K,\, \sigma_0)$ and $C_2 = C_2(C,\, \kappa)$. The parameter satisfies $\lambda\asymp \rho$ and $\lambda \ge 8\rho $.\newline
\end{theorem}

\noindent In light of the above theorem, for the case of Theorem~\ref{thm:main1} where 
\begin{align*}
Z_{M^*} = \sup_{I(f - f^*)\le M^*}|\nu_n(f) - \nu_n(f^*)|,
\end{align*}
and $\beta,\beta^*\in \mathcal{R}$ where $\mathcal{R}$ is uniformly bounded by $R$ then we have with probability at-least $1-2\exp\left[ -n\rho^2C_1 \right]-C\exp\left[ -n\rho^2C_2 \right]$,
\begin{align*}
Z_{M^*} \le  \rho \left( M^* + 2R\right).
\end{align*}

\noindent In the case of Theorem~\ref{thm:main2} where
\begin{align*}
Z_{M^*} = \sup_{|\beta - \beta^*| + I(f - f^*)\le M^*}|\nu_n(f) - \nu_n(f^*)|,
\end{align*}
we have with probability at-least $1-2\exp\left[ -n\rho^2C_1 \right]-C\exp\left[ -n\rho^2C_2 \right]$,
\begin{align*}
Z_{M^*} \le \rho M^*.\newline
\end{align*}

\noindent To prove Theorem~\ref{lemma:Emp-Process}, we use a few technical lemmas from \cite{vandegeer2000empirical} namely Lemma 8.2 and Corollary 8.3; for the sake of completeness we state these lemmas in Appendix~\ref{app:vandeGeer}. 
%For proving \textbf{Case 3}, we require a slight generalization of of Lemma~8.4 of \cite{vandegeer2000empirical} which we state and prove in Appendix~\ref{app:vandeGeer}. 


\begin{proof}[\textbf{Proof of Theorem~\ref{lemma:Emp-Process}}]
We begin by noting that for any arbitrary function we have
\begin{align*}
\nu_n(f) = (\mathbb{P}_n - \mathbb{P})(-\ell(f)) = \frac{1}{n}\sum_{i=1}^{n}\left[ aY_if(\bs{x}_i) + b(f(\bs{x}_i))\right] - \mathbb{E}\left[ \frac{1}{n}\sum_{i=1}^{n}aY_if(\bs{x}_i) + b(f(\bs{x}_i)) \right].
\end{align*}
Since we assume the covariates $\bs{x}_1,\ldots, \bs{x}_n$ are fixed we obtain 
\begin{align*}
\nu_n(f) = \frac{1}{n}\sum_{i=1}^{n}a(Y_i -\mu_i)f(\bs{x}_i) \equiv a\langle \bs{Y} - \bs{\mu}, f\rangle_n,
\end{align*}
where $\mu_i = \mathbb{E}Y_i$. Thus for additive functions $f$ and $f^*$ we obtain 
\begin{align*}
\nu_n(f) - \nu_n(f^*) &= a\langle \bs{Y} - \bs{\mu}, f - f^*\rangle_n = \frac{1}{n}\sum_{i=1}^{n} a(Y_i - \mu_i)\left[ \beta-\beta^* + \sum_{j=1}^{p}f_j(x_{ij}) - f_j^*(x_{ij}) \right]\\
&= a(\beta-\beta^*)\frac{1}{n}\sum_{i=1}^{n}(Y_i - \mu_i) + \sum_{j=1}^{p}\frac{1}{n}\sum_{i=1}^{n}a(Y_i-\mu_i)(f_j(x_{ij}) - f_j^*(x_{ij}))\\
&= a(\beta-\beta^*)(\overline{\bs{Y}} - \overline{\bs{\mu}}) + \sum_{j=1}^{p}a\langle \bs{Y} - \bs{\mu}, f_j-f_j^*\rangle_n.
\end{align*}
From now on we will assume, without loss of generality, that $|a| = 1$ since this constant is absorbed into a constant $\kappa$ which we define later.

To control the first term, $(\beta - \beta^*)(\overline{\bs{Y}} - \overline{\bs{\mu}})$, we simply apply Lemma~\ref{lemma:lemma8.2}. For the second part, we consider 2 cases. 

\noindent\textbf{Case 1: Logarithmic Entropy.} We first note that if the entropy bound holds, then the same bound holds~(upto a constant) for the class
\begin{equation}
\label{eqn:class-scaled}
\left\{\frac{f_j - f_j^*}{\|f_j - f_j^*\|_n + \lambda P_{st}(f_j - f_j^*)}: f_j\in \mathcal{F}\right\},
\end{equation}
for some $f_j^*\in \mathcal{F}$ for all $j= 1,\ldots,p$. Now we apply Lemma~\ref{lemma:cor8.3} to the above class by first noting that $R\le 1$ and then using the bound for Dudley's integral
\begin{equation}
A_0^{1/2}T_n^{1/2}\int_0^{1} \log^{1/2}\left( \frac{1}{u}  + 1\right)\, du \le \wt{A}_0T_n^{1/2},
\end{equation}
we have for all $\delta$ that satisfy
\begin{equation}
\delta\ge 2C\wt{A}_0\sqrt{\frac{T_n}{n}},
\end{equation}
where the constant $C$ depends only on $K$ and $\sigma_0$, we have
\begin{equation*}
\mathbb{P}\left( \sup_{f_j\in \mathcal{F}} \left| \frac{\frac{1}{n} \sum_{i=1}^{n}(Y_i - \mu_i)\left( f_j(x_{ij}) - f^*_j(x_{ij}) \right)}{\|f_j - f_j^*\|_n+ \lambda P_{st}(f_j - f_j^*)} \right|\ge \delta \right) \le C\exp\left[ -\frac{n\delta^2}{4C^2} \right].
\end{equation*}
We can now take $\delta = \rho  \ge 2C\wt{A}_0 \max\left\{ \sqrt{\frac{T_n}{n}}, \sqrt{\frac{\log p}{n}} \right\}\ge 2C\wt{A}_0\sqrt{\frac{T_n}{n}}$ which holds for all $\kappa \ge 2C\wt{A}_0$. Applying the above result with a union bound gives us
\begin{align*}
&\mathbb{P}\left( \max_{j=1,\ldots,p}\sup_{f_j\in \mathcal{F}}  \frac{\left| \langle \bs{Y} - \bs{\mu}, {f}_j - f^*_j \rangle_n\right|}{\|f_j-f_j^*\|_n +  \lambda P_{st}(f_j-f_j^*)} \ge \rho \right) \\
&\le p C\exp\left[ -\frac{n\rho^2}{4C^2} \right]= C\exp\left[ -\frac{n\rho^2}{4C^2} + \log p \right] \\
&= C\exp\left[ - n\rho^2\left( \frac{1}{4C^2} - \frac{\log p}{n\rho^2} \right)\right] \le C\exp\left[ -n\rho^2C_2 \right],
\end{align*}
for a constant $C_2>0$ that depends on $C$ and $\wt{A}_0$. To see this, note that
\begin{align*}
\frac{1}{4C^2} - \frac{\log p}{n\rho^2} = \frac{1}{4C^2} - \frac{1}{\kappa \max\left\{ \frac{T_n}{\log p}, 1 \right\}} \ge \frac{1}{4C^2} - \frac{1}{\kappa},
\end{align*}
which is positive if $\kappa> 4C^2$. Thus we can take the constant $\kappa$ such that $\kappa > \max\left\{ 4C^2, 2C\wt{A}_0 \right\}$. Hence $\kappa$ depends on $C(K,\sigma_0)$ and $\wt{A}_0(A_0)$.


\noindent\textbf{Case 2: Polynomial Entropy with Smoothness.} Now we note that same entropy bound holds for the class 
\begin{equation}
\label{eqn:class-scaled2}
\wt{\mathcal{F}} = \left\{\frac{f_j - f_j^*}{\|f_j - f_j^*\|_n + \lambda P_{st}(f_j - f_j^*)}: f_j\in \mathcal{F}\right\},
\end{equation}
and we can now apply Lemma~\ref{lemma:cor8.3} by noting that 
\begin{align*}
\int_{0}^{1} H^{1/2}(u, \wt{\mathcal{F}}, Q_n)\, du \le \wt{A}_0\lambda^{-\alpha/2},
\end{align*}
for some constant $\wt{A}_0 = \wt{A}_0(A_0)$. For some $C = C(K,\sigma_0)$ and all
$\delta\ge 2C\wt{A}_0\lambda^{-\alpha/2}n^{-1/2}$ 
we have 
\begin{align}
\label{eqn:lemmaUse}
\mathbb{P}\left( \sup_{f_j\in \mathcal{F}}  \frac{\left| \langle \bs{Y} - \bs{\mu}, {f}_j - f^*_j \rangle_n\right|}{ \|f_j-f_j^*\|_n + \lambda P_{st}(f_j-f_j^*) } \ge \delta \right) \le C\exp\left[ -\frac{n\delta^2}{4C^2} \right].
\end{align}
Since $\lambda \ge \rho$ we note that $2C\wt{A}_0\lambda^{-\alpha/2}n^{-1/2} \le 2C\wt{A}_0\rho^{-\alpha/2}n^{-1/2}$ and that 
\begin{align*}
2C\wt{A}_0\rho^{-\alpha/2}n^{-1/2} \le \rho \Leftrightarrow \rho \ge \left( 2C\wt{A}_0 \right)^{\frac{2}{2+\alpha}} n^{-\frac{1}{2+\alpha}}.
\end{align*}
Which holds by definition since $\rho = \kappa\max\left( \sqrt{\frac{\log p}{n}}, n^{-\frac{1}{2+ \alpha}} \right) \ge \kappa n^{-\frac{1}{2+\alpha}}$ and $\kappa$ is sufficiently large
(any $ \kappa \ge \left( 2C\wt{A}_0 \right)^{\frac{2}{2+\alpha}}$ would suffice). Therefore, we can take $\delta = \rho$ in \eqref{eqn:lemmaUse} along with a union bound to obtain 
\begin{align*}
\mathbb{P}\left( \max_{j=1,\ldots,p}\sup_{f_j\in \mathcal{F}}  \frac{\left| \langle \bs{Y} - \bs{\mu}, {f}_j - f^*_j \rangle_n\right|}{ \|f_j-f_j^*\|_n + \lambda P_{st}(f_j-f_j^*) } \ge {\rho} \right) &\le pC\exp\left[ - \frac{n\rho^2}{4C^2} \right]\\
&= C\exp\left[ - n\rho^2\left( \frac{1}{4C^2} - \frac{\log p}{n\rho^2} \right)\right]\\
&\le C\exp\left[ - n\rho^2C_2 \right],
\end{align*}
for some positive constant $C_2 = C_2(C,\wt{A}_0)$ exactly as in Case 1. 


%\noindent\textbf{Case 3: Mixed entropy bounds.} We know from the previous 2 cases that

\end{proof}







==> sections/app_proofVandeGeer.tex <==

\section{Some Results from \cite{vandegeer2000empirical} }
\label{app:vandeGeer}

\begin{lemma}[Lemma 8.2 of \cite{vandegeer2000empirical}]
\label{lemma:lemma8.2}
Suppose that $Y_1-\mu_1,\ldots, Y_n-\mu_n$ are mean zero sub-Gaussian random variables, i.e., they satisfy \eqref{eqn:subGaussian}. Then for all $\gamma\in \mathbb{R}^n$ and $\rho>0$, 
\begin{equation}
\mathbb{P}\left( \left| \sum_{i=1}^{n}(Y_i-\mu_i)\gamma_i \right| \ge \rho \right) \le 2\exp\left[ -\frac{\rho^2}{8(K^2+\sigma_0^2)\sum_{i=1}^{n}\gamma_i^2} \right],
\end{equation}
in particular if $\gamma_i = 1/n$ then we have 
\begin{equation}
\mathbb{P}\left( \left| \frac{1}{n}\sum_{i=1}^{n}Y_i-\mu_i \right| \ge \rho \right) \le 2\exp\left[ -\frac{n\rho^2}{8(K^2+\sigma_0^2)} \right].
\end{equation}

\end{lemma}


\begin{lemma}[Corollary 8.3 of \cite{vandegeer2000empirical}]
\label{lemma:cor8.3}
Suppose that $\sup_{f_j\in \mathcal{F}}\|f_j\|_n \le R$ for a univariate function class $\mathcal{F}$ and that $Y_1-\mu_1,\ldots, Y_n-\mu_n$ are mean zero sub-Gaussian random variables, i.e. they satisfy \eqref{eqn:subGaussian}. Then for some constant $C = C(K,\sigma_0)$, and for all $\delta>0$ satisfying 
\begin{equation}
\sqrt{n}\delta \ge 2C\left( \int_{0}^{R}H^{1/2}(u, \mathcal{F},Q_n) \, du \vee R\right),
\end{equation}
we have 
\begin{equation}
\mathbb{P}\left( \sup_{f_j\in \mathcal{F}} \left| \frac{1}{n}\sum_{i=1}^{n}(Y_i-\mu_i)f_j(x_{ij}) \right|\ge \delta \right) \le C\exp\left[ -\frac{n\delta^2}{4C^2R^2} \right].
\end{equation}
\end{lemma}

%\begin{lemma}[Lemma 8.4 of \cite{vandegeer2000empirical}]
%\label{lemma:lemma8.4}
%Suppose that $\sup_{f_j\in \mathcal{F}}\|f_j\|_n \le R$ for a univariate function class $\mathcal{F}$ and that $Y_1-\mu_1,\ldots, Y_n-\mu_n$ are mean zero sub-Gaussian random variables, i.e. they satisfy \eqref{eqn:subGaussian}. Further assume that 
%\begin{equation}
%H(\delta, \mathcal{F}, Q_n) \le A_0\delta^{-\alpha},
%\end{equation}
%for $\alpha\in (0,2)$. Then for some constant $C = C(A_0,\alpha, R,K,\sigma_0)$ we have for all $T\ge C$,
%\begin{equation}
%\mathbb{P}\left( \sup_{f_j\in \mathcal{F}} \frac{\left|\frac{1}{n}\sum_{i=1}^{n}(Y_i-\mu_i)f_j(x_{ij}) \right|}{\|f_j\|_n^{1-\alpha/2}}\ge \frac{T}{\sqrt{n}} \right) \le C\exp \left[ -\frac{T^2}{C^2} \right].
%\end{equation}
%\end{lemma}
%
%
%
%
%
%%\begin{lemma}
%%\label{lemma:lemma8-4}
%%Assume that $\sup_{f\in \mathcal{F}}\|f\|_{Q_n} \le R$ for some univariate function class $\mathcal{F}$. Further assume the entropy bound
%%\begin{equation}
%%H(\delta,\, \mathcal{F},\, Q_n) \le A_0 (\delta\gamma)^{-\alpha},\ 
%%\end{equation}
%%for some $\alpha \in (0,\, 2)$ and constant $A_0$ and that 
%%\begin{equation}
%%\max_{i=1,\ldots, n} K^2\left( \mathbb{E} e^{\e_i^2/K^2}-1\right)\le \sigma_0^2,
%%\end{equation}
%%for mean zero random variables $\e_i$. Then for some constant $C = C(A_0,\alpha,K,\sigma_0)$, we have for all $T\ge C,$
%%\begin{equation}
%%P\left( \sup_{f\in \mathcal{F}} \frac{\left| \frac{1}{n}\sum_{i=1}^{n}\e_if(x_i)  \right|}{\|f\|_{Q_n}^{1-\alpha/2}} \ge T \frac{\gamma^{-\alpha/2}}{\sqrt{n}} \right) \le C\exp\left( -\frac{T^2\gamma^{-\alpha}}{C^2} \right).
%%\end{equation}
%%\end{lemma}
%%
%%\begin{proof}
%%We have
%%\begin{align*}
%%\int_{0}^{\delta} H^{1/2}(u,\mathcal{F}, Q_n)\, du \le \wt{A}_0\gamma^{-\alpha/2}\delta^{1-\alpha/2}.
%%\end{align*}
%%For $C_1\ge 1$ by Corollary 8.3 of \cite{vandegeer2000empirical} we have,
%%\begin{align*}
%%\mathbb{P}\left( \underset{f\in \mathcal{F}, \|f\|_{Q_n} \le \delta}{\sup} \left|\frac{1}{n} \sum_{i=1}^{n} \e_if(x_i)\right|\ge 2cC_1\wt{A}_0\frac{\gamma^{-\alpha/2}}{\sqrt{n}}\delta^{1-\alpha/2} \right) \le c\exp\left( -C_1^2\wt{A}_0^2\delta^{-\alpha}\gamma^{-\alpha} \right),
%%\end{align*}
%%for some constant $c = c(K, \sigma_0)$.
%%Now we apply the peeling device (see \cite{vandegeer2000empirical}) to the class $\mathcal{F}$. Let $T = 2cC_1A_12^{1-\alpha/2}$,
%%\begin{align*}
%%\mathbb{P}&\left( \underset{f\in \mathcal{F}}{\sup }    \frac{ \left|\frac{1}{{n}} \sum_{i=1}^{n} \e_if(x_i)\right|}{\|f\|_{Q_n}^{1-\alpha/2}}\ge T\frac{\gamma^{-\alpha/2}}{\sqrt{n}} \right)= \mathbb{P}\left( \bigcup_{s=1}^{\infty}\sup_{f:f\in \mathcal{F}, \frac{ R }{2^s}\le \|f\|_{Q_n}\le \frac{R}{2^{s-1}} } \frac{\left|\frac{1}{{n}} \sum_{i=1}^{n} \e_if(x_i)\right|}{\|f\|_{Q_n}^{1-\alpha/2}}\ge T\frac{\gamma^{-\alpha/2}}{\sqrt{n}} \right) \\
%%&\le \sum_{s=1}^{\infty}\mathbb{P}\left( \sup_{f:f\in \mathcal{F}, \|f\|_{Q_n}\le \frac{R}{2^{s-1}} } {\left|\frac{1}{{n}} \sum_{i=1}^{n} \e_if(x_i)\right|} \ge T\frac{\gamma^{-\alpha/2}}{\sqrt{n}}\left( \frac{R}{2^s} \right)^{1-\alpha/2} \right)\\
%%&= \sum_{s=1}^{\infty}\mathbb{P}\left( \sup_{f:f\in \mathcal{F}, \|f\|_{Q_n}\le \frac{R}{2^{s-1}} } {\left|\frac{1}{{n}} \sum_{i=1}^{n} \e_if(x_i)\right|} \ge \frac{T\gamma^{-\alpha/2}}{\sqrt{n}2^{1-\alpha/2}}\left( \frac{R}{2^{s-1}} \right)^{1-\alpha/2} \right)\\
%%&= \sum_{s=1}^{\infty}\mathbb{P}\left( \sup_{f:f\in \mathcal{F}, \|f\|_{Q_n}\le \frac{R}{2^{s-1}} } {\left|\frac{1}{{n}} \sum_{i=1}^{n} \e_if(x_i)\right|} \ge {2cC_1A_1\frac{\gamma^{-\alpha/2}}{\sqrt{n}} }\left( \frac{R}{2^{s-1}} \right)^{1-\alpha/2} \right)\\
%%&\le \sum_{s=1}^{\infty} c\exp\left\{ -C_1^2\wt{A}_0^2\gamma^{-\alpha} \left( \frac{R}{2^{s-1}} \right)^{-\alpha} \right\}= \sum_{s=1}^{\infty} c\exp\left\{ -C_1^2A_1^2\left( 2^{-s+1} \right)^{-\alpha}R^{-\alpha} \gamma^{-\alpha}\right\} \\
%%&\le C\exp\left(-\frac{T^2\gamma^{-\alpha}}{C^2}\right).
%%\end{align*}
%%\end{proof}
%%


==> sections/extra.tex <==
% !TeX root = ../MANUSCRIPT.tex

%\section{Structural Penalty Details}
\subsection{Semi-norms vs Squared Semi-norms}
\label{sec:Insights}
For a semi-norm $P_{semi}$, using $P_{st} = P_{semi}^2$ in \eqref{eq:unif-sparse-add1} can give poor theoretical performance (as noted in \cite{meier2009high} for case of $P_{semi} = P_{sobolev}$) and, can also be computationally expensive (as disscussed in Section~\ref{sec:Algorithm}). In this subsection, we show a surprising result: using a squared semi-norm penalty does not actually lead to a sparse solution. 

To be precise, using $P_{st} = P_{semi}^2$ leads to an active set ${S} = \{j: \wh{f}_j \not\equiv 0\}$, for which either $|{S}| = 0$ or $|{S}| = p$; in contrast, using $P_{st} = P_{semi}$ can give active sets such that $0<|{S}|<p$. To demonstrate this phenomenon, we consider first the univariate problem 
\begin{align}
\label{eq:univ1}
\wh{f}_1 \gets \underset{f\in \mathcal{F}}{\operatorname{argmin}}\  \frac{1}{n}\sum_{i=1}^n \left(y_i - f\left(x_{i}\right)\right)^2 + \lambda_{st} P^2_{semi}\left(f\right) + \lambda_{sp}\left\|f\right\|_n,
\end{align}
and characterize conditions for when $\wh{f}_1\equiv 0$. Recall that $\wh{f}_1$ minimizes the objective in \eqref{eq:univ1} if for every direction $h$, the objective is minimized at $\e = 0$ along the path $\wh{f}_1 + \e h$. In the following lemma, we state necessary and sufficient conditions for $\wh{f}_1$ to be $\bs{0}$ (proof in Appendix~\ref{app-sec:ProofSec2}). 
\begin{lemma}
	\label{lemma:univ1}
For $\wh{f}_1$ defined by \eqref{eq:univ1}, the following are equivalent: (a) $\wh{f}_1 = \bs{0}$, (b) for every direction $h$, $\left|{n^{-1}}\sum_i y_i {h(x_i)}/{\left\|h\right\|_n}\right| \leq \lambda_{sp}$, (c) $\|\bs{y}\|_n\le \lambda_{sp}$.
\end{lemma}
Condition (c) of Lemma~\ref{lemma:univ1} is problematic when we consider multiple features in our additive problem \eqref{eq:unif-sparse-add1}. For additive models, condition (c) implies that sparsity of component $\wh{f}_j$, does not depend on covariate $j$. Thus if all smoothing penalties are squared semi-norms then for a given $\lambda_{sp}$, either all $\wh{f}_j = {\bf 0}$ or all $\wh{f}_j\not = {\bf 0}$. 

On the other hand, consider the optimization problem 
 \begin{equation}\label{eq:univ2}
 \wh{f}_2 \gets \underset{f\in \mathcal{F}}{\operatorname{argmin}}\  \frac{1}{n}\sum_{i=1}^n \left(y_i - f\left(x_{i}\right)\right)^2 + \lambda_{st} P_{semi}\left(f\right) + \lambda_{sp}\left\|f\right\|_n,
 \end{equation}
 then we have the following lemma~(proof in Appendix~\ref{app-sec:ProofSec2}).
 
 \begin{lemma}
 		\label{lemma:univ2}
 		For $\wh{f}_2$ defined by \eqref{eq:univ2}, the following are equivalent: (a) $\wh{f}_2 = \bs{0}$, (b) for every direction $h$, there exists some $V\in [-1,1]$ such that $\Big|{n^{-1}}\sum_i y_i {h(x_i)}/{\|h\|_n} - \lambda_{st}{VP_{semi}(h)}/{\|h \|_n}\Big| \leq \lambda_{sp}$. 
 		
 		Additionally, if $\|\bs{y}\|_n \le \lambda$ then $\wh{f}_2=\bs{0}$, but the converse is not necessarily true. 
 \end{lemma}
Unlike the squared semi-norm penalties, conditions for $\wh{f}_2 = \bs{0}$ involve the feature vector $\bs{x}$. Thus for an additive model the sparsity of component $j$ depends on both the response vector $\bs{y}$, and $j$-th covariate $(x_{1j}, \ldots, x_{nj})$. Consequently, there are many $(\lambda_{sp}, \lambda_{st})$ pairs for which we will have some $\wh{f}_j = {\bf 0}$ and some $\wh{f}_j \not = {\bf 0}$. Additionally, Lemma~\ref{lemma:univ2} gives us a conservative value for $\lambda_{max} = \|\bs{y}\|_n$, i.e., the $\lambda_{sp}$ value for which all $\wh{f}_j = \bs{0}$.



==> sections/extraApp.tex <==
% !TeX root = ../Appendix.tex

\section{Block Coordinate Descent Algorithm and Additional Figures}
\label{app:AdditionalFigures}

\noindent Algorithm~\ref{alg:additiveBC} is the block coordinate descent algorithm that can be used to estimate \name s.\newline

\noindent Figure~\ref{fig:SamplePlots} shows estimated functions for SpAM with 3,10 and 30 basis functions, and for SSP.\newline


\noindent Figure~\ref{fig:SamplePlots2} shows estimated functions  for trend filtering of orders $k=0,1,2$.\newline 



\noindent Figure~\ref{fig:DataAnalysisExample} shows estimated functions for the various methods for the analysis of Boston housing data,

\begin{algorithm}
	\caption{Block Coordinate Descent for Least Squares Loss}
	\label{alg:additiveBC}
	\begin{algorithmic}[1]
		\State Initialize $f^{0}_1,\ldots f^{0}_p \gets {\bf 0}, \beta^0 \gets 0$, $\bs{r}\gets \bs{y}$, $k\gets 1$
		\While{$k\le max\_iter$ \textbf{ and } not converged} 
		
		\State Update 
		\begin{align*}
		\beta^k \gets n^{-1}\sum_{i=1}^{n}r_i,% n^{-1}\sum_{i=1}^{n}\Big( y_i - \sum_{j=1}^pf_j^{k-1}(x_{ij}) \Big).
		\quad \bs{r} \gets \bs{r} - \beta^k\bs{1}.
		\end{align*}
		\For{$ j = 1,\, \ldots,\, p$} 
		\State Set $\bs{r}_{-j}$ as
		\[{r}_{-j,i} = r_i + f_j^{k-1}(x_{ij}). \]
		
		\State Update 
		\[
		f^{k}_j \gets \Big(1 - {t\lambda}/{\|f^{inter}_j\|_n}\Big)_{+}f^{inter}_j,
		\]		
		\ \ \ \ \ \ \ \ \ where 
		\begin{equation}\label{eq:updateBC}
		f^{inter}_j \gets \underset{f\in \mathcal{F}}{\operatorname{argmin }}\ \frac{1}{2} \Big\| \bs{r}_{-j} - f\Big\|_n^2 + t\lambda^2 P_{st}\left(f\right).
		\end{equation}
		\State Update $\bs{r}$ to
		\begin{align*}
		r_i \gets r_{-j,i} + f^k_{j}(x_{ij}). 
		\end{align*}
		\EndFor
		\EndWhile
		\State\Return $\beta^k, f^k_1,\ldots, f^k_p$ 
		%\EndProcedure
	\end{algorithmic}
\end{algorithm}


\begin{figure}
	\centering
	\includegraphics[height = 0.23\textheight]{Plots/spam3}
	\includegraphics[height = 0.23\textheight]{Plots/spam10}
	\includegraphics[height = 0.23\textheight]{Plots/spam30}
	\includegraphics[height = 0.23\textheight]{Plots/ssp.pdf}
	\caption{Examples of estimated signal functions by SpAM~\citep{ravikumar2009sparse} and Sobolev Smoothness Penalty~\citep{meier2009high} for Scenario~4.}
	\label{fig:SamplePlots}
\end{figure}


\begin{figure}
	\centering
	\includegraphics[width = \textwidth]{Plots/tf0.pdf}
	\includegraphics[width = \textwidth]{Plots/tf1.pdf}
	\includegraphics[width = \textwidth]{Plots/tf2.pdf}
	\caption{Examples of estimated signal functions by Trend Filtering~\citep{sadhanala2017additive} for Scenario~4.}
	\label{fig:SamplePlots2}
\end{figure}




\begin{figure}
\centering
\includegraphics[scale = 0.273]{PlotsData/v1}
\includegraphics[scale = 0.273]{PlotsData/v2}
\includegraphics[scale = 0.273]{PlotsData/v3}
\includegraphics[scale = 0.273]{PlotsData/v4}
\includegraphics[scale = 0.273]{PlotsData/v5}
\includegraphics[scale = 0.273]{PlotsData/v6}
\includegraphics[scale = 0.273]{PlotsData/v7}
\includegraphics[scale = 0.273]{PlotsData/v8}
\includegraphics[scale = 0.273]{PlotsData/v9}
\includegraphics[scale = 0.273]{PlotsData/v10}
\caption{Plots of fitted functions for the original 10 covariates for a single split of the data into training and test sets for lasso~(\protect\includegraphics[height=0.5em]{PlotsData/black1.png}), SpAM~(\protect\includegraphics[height=0.5em]{PlotsData/red1.png}) with $M=3$ basis functions, SSP~(\protect\includegraphics[height=0.5em]{PlotsData/green1.png}) and, TF~(\protect\includegraphics[height=0.5em]{PlotsData/blue1.png}) of order $k=0$.} 
\label{fig:DataAnalysisExample}
\end{figure}


==> sections/proofsAdditive.tex <==
% !TeX root = Manuscript.tex

\section{Proof of Theorem \ref{thm:main}}
\label{app:proofsAdditive}

Recall that $\{\wh{f}_j\}_{j=1}^p \in \mathcal{F}$ where $\mathcal{F}$ is some arbitrary univariate function class 
%and also recall the notation $f_j = [f_j(x_{1,l}),f_j(x_{n,l}),\ldots,f_j(x_{n,l})]^T$. 
. We denote the functions $\wh{f}(\bs{x}) = \wh{c} +  \sum_{j=1}^{p}\wh{f}_j({x}_j)$ and $f^0(\bs{x}) = c^0+ \sum_{j=1}^{p}f^0_j({x}_j)$ for $\bs{x} = [x_1,\ldots,x_p]^T\in \mathbb{R}^p$. For the proof of Theorem~\ref{thm:main}, $\lambda_n$ and $\rho_n$ are functions of $n$ but for convenience we will simply write $\lambda,\, \rho$. We begin the proof of Theorem~\ref{thm:main} with a basic inequality. For a given function $\wh{f}$, we denote the excess risk by 
\begin{equation}
\mathcal{E}(\wh{f}) = \mathbb{P}\left( \ell(f^0) - \ell(\wh{f}) \right),
\end{equation}
and the empirical process term by 
\begin{equation}
\nu_n(\wh{f}) = \left( \mathbb{P}_n - \mathbb{P} \right)(-\ell(\wh{f})).
\end{equation}


\begin{lemma}[Basic Inequality]
Assume that the loss function is of the form $\ell(f(\bs{x}_i)) = aY_if(\bs{x}_i) + b(f(\bs{x}_i))$. For any function $f^* = c^*+\sum_{j=1}^{p}f_j^*$, where $f_j^*\in \mathcal{F}$ and, the solution $\wh{f}$ of (\ref{eq:prop}), we have the following basic inequality
\begin{align*}
\mathcal{E}(\wh{f}) + \lambda\sum_{j=1}^{p}\left(\|\wh{f}_j\|_n + \lambda P_{st}(\wh{f}_j)\right) &\le |a||c^* - \wh{c}|\left| \ol{\bs{Y}} - \bs{\mu} \right| + |a|\sum_{j=1}^{p}\left|  \langle \bs{Y} - \bs{\mu},  \wh{f}_j - f^*_j\rangle_n \right| \\
&+\lambda\sum_{j=1}^{p}\left(\|f^*_j\|_n + \lambda P_{st}(f^*_j)\right) + \mathcal{E}(f^*),
\end{align*}
where $\langle \bs{Y}- \bs{\mu}, f\rangle_n = \frac{1}{n}\sum_{i=1}^{n}(Y_i - \mu_i)f(\bs{x_i})$ and $\ol{\bs{Y}} = \frac{1}{n}\sum_{i=1}^{n}Y_i$.
\end{lemma}

% % % % % % % % % % % % % % % %
% % % % % % % % % % % % % % % %% BEGIN PROOF HERE
% % % % % % % % % % % % % % % %

\begin{proof}
Let $I(f) = \sum_{j=1}^{p}P_{st}(f_j) + \lambda \sum_{i=1}^{n}\|f_j\|_n$ then we have
\begin{align*}
-\mathbb{P}_n\ell\left( \wh{c} + \sum_{j=1}^{n}\wh{f}_j +  \right) + \lambda I(\wh{f}) \le -\mathbb{P}_n\ell\left( {c}^* + \sum_{j=1}^{n}{f}^*_j +  \right) + \lambda I({f}^*).
\end{align*}
By adding an subtracting the appropriate terms we obtain the inequality 
\begin{align*}
\mathcal{E}(\wh{f}) + \lambda I(\wh{f}) \le \left[ \nu_n(f^*) - \nu_n(\wh{f}) \right] + \lambda I(f^*) + \mathcal{E}(f^*).
\end{align*}
Now if we assume that 
\begin{align*}
\ell(Y_i, f(\bs{x}_i)) = aY_if(\bs{x}_i) + b(f(\bs{x}_i)),
\end{align*}
hence we have 
\begin{align*}
\nu_n(f) &= (\mathbb{P}_n - \mathbb{P})(-\ell(f)) = -\frac{1}{n}\sum_{i=1}^{n} \left[ aY_if(\bs{x}_i) + b(f(\bs{x}_i)) -  a\mathbb{E}Y_if(\bs{x}_i) - b(f(\bs{x}_i)) \right]\\
&= -a\langle \bs{Y} - \bs{\mu}, f\rangle_n,
\end{align*}
which implies that 
\begin{align*}
\nu_n(f^*) - \nu_n(\wh{f}) &= a\langle \bs{Y} - \bs{\mu}, \wh{f} - f^*\rangle_n\\
&= a\left[ \langle \bs{Y} - \bs{\mu}, \wh{c} - c^*\rangle_n + \sum_{j=1}^{p}\langle \bs{Y} - \bs{\mu}, \wh{f}_j - f^*_j\rangle_n \right].
\end{align*}


\end{proof}


\begin{lemma}[Bounding the term $|\ol{\bs{Y}} - \bs{\mu}|$]
For a mean zero random vector $\bs{\e} = [\e_1,\ldots\e_n]$ we have the following two cases:
\begin{enumerate}
\item If $\bs{\e}$ is uniformly sub-Gaussian, i.e. 
\begin{equation}
\max_i K^2\left( \mathbb{E}e^{\e_i^2/K^2} -1 \right)\le \sigma_0^2\ ,
\end{equation}
then for all $\rho>0$,
\begin{equation}
\mathbb{P} \left( |\ol{\bs{\e}}| \ge \rho \right) \le 2\exp\left[ -\frac{n\rho^2}{8(K^2+\sigma_0^2)}\right].
\end{equation}

\item If $\bs{\e}$ is uniformly sub-exponential, i.e. 
\begin{equation}
\max_i 2K^2\left( \mathbb{E}e^{\e_i/K} -1 - |\e_i|/K \right)\le \sigma_0^2\ ,
\end{equation}
then for all $\rho>0$,
\begin{equation}
\mathbb{P} \left( |\ol{\bs{\e}}| \ge \rho \right)\le 2\exp\left[ -\frac{n\rho^2}{2(\rho K + \sigma_0^2)} \right].
\end{equation}
\end{enumerate}
\end{lemma}
\begin{proof}
Part 1 and 2 follow immediately from Lemmas 8.2 and 8.6 of \cite{vandegeer2000empirical}, respectively.
\end{proof}

%\textbf{Recall Notation:} $\hd_j = \wh{f}_j-f^0_j$ and $H(\delta, \mathcal{F}, Q)$ is the $\delta$ entropy of the function class $\mathcal{F}$ with respect to the $L^2(Q)$ norm for some measure $Q$ We also define the empirical measure $Q_n$ such that $\|f\|^2_{Q_n} = \|f\|^2_n = \frac{1}{n}\sum_{i=1}^{n}[f(x_i)]^2$.

\begin{lemma}[Bounding the term $|\langle  \bs{Y} - \bs{\mu}, \wh{f} - f^*\rangle_n| $]
For $\lambda\ge 4\rho$ we have the following
\begin{enumerate}
\item For the entropy bound
\begin{equation}
H(\delta, \{f\in \mathcal{F}:\|f\|_n\le 1 \}, Q_n) \le A_0\delta^{-\alpha},
\end{equation} 

\end{enumerate}
 where $\rho = \kappa\max\left( n^{-\frac{1}{2+\alpha}},\, \sqrt{\frac{\log p}{n}} \right)$ and for some constant $\kappa$, if
we then have with probability at least $1-c_2\exp\left(-c_3n\rho^2\right)$
\begin{equation}
|\langle \e,\wh{f}_j - f^*_j\rangle_n|\le \rho \|\wh{f}_j - f^*_j\|_n + \rho\lambda \up(\wh{f}_j - f^*_j),
\end{equation}
for all $j=1,\ldots,p$ and positive constants $c_2$ and $c_3$.
\end{lemma}

\begin{proof}
Firstly, for $\mathcal{F}_0 = \{f\in \mathcal{F}: \up(f)\le 1\}$ we have by assumption a $\delta$ cover $f_1,\ldots,f_N$ such that for all $f\in \mathcal{F}_0$ we have $
\min_{j\in \{1,\ldots,N\}} \| f_j -  f\|_n\le \delta$. Now we are interested in the set $\mathcal{F}_{0,\lambda} = \{f\in \mathcal{F}: \lambda\up(f)\le 1\}$.
%Firstly, we note that $\{\lambda f : f\in \mathcal{F}\text{ and } \up(f) \le 1\} \subset \mathcal{F}_{0,\lambda}$. 
Firstly, for a function $f\in \mathcal{F}_{0,\lambda}$,
\begin{align*}
\min_{j\in \{1,\ldots,N\}} \| f - f_j/\lambda\|_n = \min_{j\in \{1,\ldots,N\}} \frac{1}{\lambda}\| \lambda f - f_j\|_n\le  \frac{\delta}{\lambda},
\end{align*}
because $\up(\lambda f) = \lambda \up(f) \le 1\Rightarrow  \lambda f \in \mathcal{F}_0$. This means that the set $\{f_1/\lambda,\ldots, f_N/\lambda\}$ is a $\de/\lambda$ cover of the set $\mathcal{F}_{0,\lambda}$.

This implies that $H(\delta, \mathcal{F}_0,Q_n) \le A_0\delta^{-\alpha}\Rightarrow H(\delta/\lambda, \mathcal{F}_{0,\lambda},Q_n) \le A_0\delta^{-\alpha}$ or equivalently $H(\delta, \mathcal{F}_{0,\lambda}, Q_n) \le A_0(\delta\lambda)^{-\alpha}$. Finally, since $\{f\in\mathcal{F}: I(f)\le 1\} \subset \{f\in\mathcal{F}: \up(f)\le \lambda^{-1}\}$ we have 
\begin{align*}
H(\delta, \{f\in \mathcal{F}: I(f)\le 1 \}, Q_n) \le A_0(\delta\lambda)^{-\alpha} \le A_1(\delta\rho)^{-\alpha},
\end{align*}
since $\lambda^{-1}\le \rho^{-1}/4$.

We now apply Lemma~\ref{lemma:lemma8-4} to the class $\left\{ \frac{{f}}{I({f} )}: {f}\in \mathcal{F} \right\}$ with $T = \sqrt{n}\rho^{1+\alpha/2}$. We have  for $\kappa> c_2$ sufficiently large
\begin{align*}
P\left(\sup_{f_j\in \mathcal{F}} \frac{\left| \frac{1}{n} \sum_{i=1}^{n}\e_if_j(x_i) \right|}{\|f_j\|_n^{1-\alpha/2} I^{\alpha/2}(f_j)} \ge \rho \right)\le c_2\exp\left( -\frac{n\rho^{2}}{c_2^2} \right),
\end{align*}
and by the union bound we have
\begin{align*}
P\left(\max_{j\in \{1,\ldots,p\}}\sup_{f_j\in \mathcal{F}} \frac{\left| \langle\e, f_j\rangle_n \right|}{\|f_j\|_n^{1-\alpha/2} I^{\alpha/2}(f_j)} \ge \rho \right) &\le pc_2\exp\left( - \frac{n\rho^{2} }{c_2^2}\right)  \\
&\le c_2\exp\left( - \frac{n\rho^{2}  }{c_2^2}+\log p \right) \\
&= c_2\exp\left\{ - n\rho^2\left( \frac{1}{c_2^2} - \frac{\log p }{n\rho^2}\right) \right\}\\
&\le c_2\exp\left( -c_3n\rho^2 \right),
\end{align*}
for some constant $c_3\ge  \frac{1}{c_2^2} - \frac{\log p }{n\rho^2}$. Finally, we show that $c_3> 0$. This follows from the fact that $ \frac{1}{c_2^2} - \frac{\log p }{n\rho^2}> 0\Leftrightarrow n\rho^2 > c_2^2\log p$. This holds since $n\rho^2\ge \kappa^2\log p$ and $\kappa> c_2$. Thus, we have with probability at least $1-c_2\exp\left(c_3n\rho^2\right)$ for all $j\in \{1,\ 2,\ \ldots,\ p\}$
\begin{align*}
|\langle\e,\wh{f}_j - f^*_j\rangle_n| \equiv |\langle\e,\hd_j\rangle_n| &\le  \rho \|\hd\|_n^{1-\alpha/2}I^{\alpha/2}(\hd_j) \\
&= \rho \|\hd_j\|_n\left\{ 1 + \frac{\lambda\up(\hd_j)}{\|\hd_j\|_n} \right\}^{\alpha/2}\le \rho \|\hd_j\|_n + \rho\lambda\up(\hd_j)\ , 
\end{align*}
where the last inequality follows by Bernoulli's inequality.
\end{proof}

\subsection{Using the Active Set}

So far we have shown that, for $\lambda\ge 4\rho$, with probability at least $1-2\exp\left(-\frac{n\rho}{c_1}\right) -c_2\exp\left(-c_3n\rho^2\right)$, the following inequality holds
\begin{align*}
\|\wh{f} - f^0\|_n^2 + 2\lambda\sum_{j=1}^{p}I(\wh{f}_j) &\le 2|\langle \e, \wh{f}-f^* \rangle_n| + 2|\bar{\e}|\sum_{j=1}^p \|\hd_j\|_n + 2\lambda \sum_{j=1}^{p}I(f^*_j)+\|f^*-f^0\|_n^2 \\
&\le \left\{ \sum_{j=1}^{p} 2\rho\|\hd_j\|_n + 2\rho\lambda\up(\hd_j)\right\}  + \left\{ 2\rho \sum_{j=1}^{p}\|\hd_j\|_n \right\} \\
&+ \left\{ 2\lambda \sum_{j=1}^{p}I(f^*_j)\right\}+\|f^*-f^0\|_n^2\\
\Rightarrow \|\wh{f}-f^0\|_n^2 + 2\lambda\sum_{j=1}^{p}I(\wh{f}_j)  &\le \sum_{j=1}^{p} \left\{ \lambda \|\hd_j\|_n + \frac{\lambda^2}{2} \up(\hd_j) + 2\lambda\|f^*_j\|_n+2\lambda^2\up(f^*_j)\right\} + \|f^* - f^0\|_n^2.
\end{align*}
For notational convenience we will exclude the $\|f^*-f^0\|_n^2$ term in the following manipulations. If $S$ is the active set then we have on the right hand side,
\begin{align*}
\mathrm{RHS} &= \lambda \sum_{j\in S} \left\{\|\hd_j\|_n +  \frac{\lambda}{2}\up(\hd_j) +2\|f^*_j\|_n + 2\lambda\up(f^*_j) \right\}+\lambda\sum_{j\in S^c} \left\{\|\wh{f}_j\|_n+\frac{\lambda}{2}\up(\wh{f}_j)\right\}\\
&\le \lambda \sum_{j\in S} \left\{\|\hd_j\|_n +  \frac{\lambda}{2}\up(\hd_j) +2\|\hd_j\|_n+2\|\wh{f}_j\|_n + 2\lambda\up(f^*_j) \right\}+\lambda\sum_{j\in S^c} \left\{\|\wh{f}_j\|_n+\frac{\lambda}{2}\up(\wh{f}_j)\right\}\\
&= 3\sum_{j\in S}\lambda\|\hd_j\|_n+2\sum_{j\in S}\lambda^2\up(f^*_j)+ \sum_{j\in S^c}\lambda\|\wh{f}_j\|+\frac{1}{2}\sum_{j\in S^c}\lambda^2\up(\wh{f}_j) + 2\sum_{j\in S}\lambda\|\wh{f}_j\|_n + \frac{1}{2}\sum_{j\in S}\lambda^2\up(\hd_j),
\end{align*}
where the inequality holds by the decomposition $\|f^*_j\|_n = \|f^*_j-\wh{f}_j+\wh{f}_j\|_n\le \|\hd_j\|_n + \|\wh{f}_j\|_n$.


\noindent On the left hand side we have
\begin{align*}
\mathrm{LHS} &= \|\wh{f} - f^0\|_n^2+2\lambda\sum_{j\in S} \left\{\|\wh{f}_j\|_n+\lambda\up(\wh{f}_j)\right\} + 2\lambda\sum_{j\in S^c} \left\{\|\wh{f}_j\|_n+\lambda\up(\wh{f}_j)\right\}\\
&\ge \|\wh{f} - f^0\|_n^2+2\lambda\sum_{j\in S} \left\{\|\wh{f}_j\|_n +\lambda\up(\hd_j)-\lambda\up(f^*_j)\right\} + 2\lambda\sum_{j\in S^c} \left\{\|\wh{f}_j\|_n+\lambda\up(\wh{f}_j)\right\},
\end{align*}
where the inequality follows from the triangle inequality $  \up(\wh{f}_j) + \up(f^*_j)\ge \up(\hd_j)$ since $\up(\cdot)$ is a semi-norm. By re-arranging the terms we obtain the inequality
\begin{equation*}
%\small
\|\wh{f} - f^0\|_n^2 + \lambda\sum_{j\in S^c}\left\{ \|\wh{f}_j\|_n + \frac{3\lambda^2}{2}\up(\wh{f}_j) \right\} + \frac{3\lambda^2}{2}\sum_{j\in S}\up(\hd_j) \le 3 \lambda\sum_{j\in S} \|\hd_j\|_n + {4\lambda^2} \sum_{j\in S}\up(f^*_j) + \|f^*-f^0\|_n^2
\end{equation*}
which implies that 
\begin{equation}
\label{eqn:inequalitySlowRates2}
\|\wh{f} - f^0\|_n^2 + \lambda\sum_{j\in S^c} \|\hd_j\|_n + \frac{3\lambda^2}{2}\sum_{j\in S}\up(\hd_j) \le 3 \lambda\sum_{j\in S} \|\hd_j\|_n + {4\lambda^2} \sum_{j\in S}\up(f^*_j) + \|f^*-f^0\|_n^2.
\end{equation}
This implies the slow rates for convergence for $\lambda \ge 4\rho$ and $s = |S|$
\begin{equation}
\label{eqn:inequalitySlowRates3}
\frac{1}{2}\|\wh{f} - f^0\|_n^2 + \le s\lambda\left\{ 3R + 2\lambda\max_{j}\up(f^*_j)\right\}  + \frac{1}{2}\|f^*-f^0\|_n^2.
\end{equation}

This completes the proof of Theorem~\ref{main-thm:thm1}. In the next section we prove the oracle inequality with fast rates via the compatibility condition.

\subsection{Using the Compatibility Condition}
\label{sec:compatibility}


Recall the compatibility condition for $f = \sum_{j=1}^{p}f_j$, whenever
\begin{equation}
\label{eqn:compatibility1}
\sum_{j\in S^c}\|f_j\|_n %+ \frac{3\lambda}{2}\sum_{j\in S}\up(f_j) 
\le 4\sum_{j\in S} \|f_j\|_n,
\end{equation}
then we have 
\begin{equation}
\sum_{j\in S}\|f_j\|_n \le \sqrt{s}\|f\|_n/\phi(S).
\end{equation}
Once we assume the compatibility condition we can prove Corollary~\ref{main-thm:additiveFastRates} by considering the following two cases.

\noindent \textbf{Case 1:} $\lambda\sum_{j\in S}\|\hd_j\|_n\ge 4\lambda^2\sum_{j\in S}\up(f^*_j)$ in which case we have
\begin{align*}
\|\wh{f} - f^0\|_n^2 + \lambda\sum_{j\in S^c} \|\hd_j\|_n + \frac{3\lambda^2}{2}\sum_{j\in S}\up(\hd_j) &\le 4 \lambda \sum_{j\in S} \|\hd_j\|_n + \|f^* - f^0\|_n^2 \ ,
\end{align*}
hence for the function $\wh{f} - f^* = \sum_{j=1}^{p}{\hd}_j$ (\ref{eqn:compatibility1}) holds and hence by the compatibility condition we have
\begin{align*}
\|\wh{f} - f^0\|_n^2 &+ \lambda\sum_{j\in S^c} \|\hd_j\|_n + \frac{3\lambda^2}{2}\sum_{j\in S}\up(\hd_j) \le \frac{4\lambda \sqrt{s}}{\phi(S)}\|\wh{f} - f^*\|_n + \|f^* - f^0\|_n^2 \\
&\le \frac{4\lambda \sqrt{s}}{\phi(S)}\|\wh{f} - f^0\|_n + \frac{4\lambda \sqrt{s}}{\phi(S)}\|{f}^* - f^0\|_n + \|f^* - f^0\|_n^2\\
&\le 2\left\{ \frac{2\lambda \sqrt{2s}}{\phi(S)} \right\}\left( \frac{\|\wh{f} - f^0\|_n}{\sqrt{2}} \right) + 2\left\{\frac{2\lambda \sqrt{s}}{\phi(S)} \right\} \left(\|{f}^* - f^0\|_n\right) + \|f^* - f^0\|_n^2\\
&\le  \frac{4\lambda^2 (2s) }{\phi^2(S)} + \frac{\|\wh{f} - f^0\|^2_n}{2}  + \frac{4\lambda^2 {s}}{\phi^2(S)} + \|{f}^* - f^0\|^2_n + \|f^* - f^0\|_n^2\\
&\le \frac{12\lambda^2 s }{\phi^2(S)}+\frac{\|\wh{f} - f^0\|^2_n}{2}  +2\|{f}^* - f^0\|^2_n,
\end{align*}
where we use the inequality $2ab\le a^2+b^2$ and this implies that 
\begin{equation}
\frac{1}{2} \|\wh{f} - f^0\|_n^2 + \lambda\sum_{j\in S^c} \|\hd_j\|_n + \frac{3\lambda^2}{2}\sum_{j\in S}\up(\hd_j) \le \frac{12s\lambda^2}{\phi^2(S)} + 2\|f^* - f^0\|_n^2.
\end{equation}

\noindent \textbf{Case 2:} $\lambda\sum_{j\in S}\|\hd_j\|_n\le 4\lambda^2\sum_{j\in S}\up(f^*_j)$ in which case we have 
\begin{align*}
\|\wh{f} - f^0\|_n^2 + \lambda\sum_{j\in S^c} \|\hd_j\|_n + \frac{3\lambda^2}{2}\sum_{j\in S}\up(\hd_j) &\le 16 \lambda^2\sum_{j\in S} \up(f^*_j) + \|f^*-f^0\|_n^2 \\
&\le 16s\lambda^2\max_{j}\up(f^*_j) + \|f^*-f^0\|_n^2,
\end{align*}
which implies
\begin{align}
\frac{1}{2}\|\wh{f} - f^0\|_n^2 + \lambda\sum_{j\in S^c} \|\hd_j\|_n + \frac{3\lambda^2}{2}\sum_{j\in S}\up(\hd_j) 
&\le 16s\lambda^2\max_{j}\up(f^*_j) + 2\|f^*-f^0\|_n^2.
\end{align}







